Short-lived High-volume Multi-A(rmed)/B(andits) Testing

Modern platforms leverage randomized experiments to make informed decisions from a given set of items (``treatments''). As a particularly challenging scenario, these items may (i) arrive in high volume, with thousands of new items being released per hour, and (ii) have short lifetime, say, due to the item's transient nature or underlying non-stationarity that impels the platform to perceive the same item as distinct copies over time. Thus motivated, we study a Bayesian multiple-play bandit problem that encapsulates the key features of the multivariate testing (or ``multi-A/B testing'') problem with a high volume of short-lived arms. In each round, a set of $k$ arms arrive, each available for $w$ rounds. Without knowing the mean reward for each arm, the learner selects a multiset of $n$ arms and immediately observes their realized rewards. We aim to minimize the loss due to not knowing the mean rewards, averaged over instances generated from a given prior distribution. We show that when $k = O(n^\rho)$ for some constant $\rho>0$, our proposed policy has $\tilde O(n^{-\min \{\rho, \frac 12 (1+\frac 1w)^{-1}\}})$ loss on a sufficiently large class of prior distributions. We complement this result by showing that every policy suffers $\Omega (n^{-\min \{\rho, \frac 12\}})$ loss on the same class of distributions. We further validate the effectiveness of our policy through a large-scale field experiment on {\em Glance}, a content-card-serving platform that faces exactly the above challenge. A simple variant of our policy outperforms the platform's current recommender by 4.32\% in total duration and 7.48\% in total number of click-throughs.

==> field_xp_analysis_old.tex <==
We now present a detailed statistical analysis of the field experiment, including  a bootstrapping \hypo\ testing and  a Difference-in-Differences (DID) analysis. 
Our analysis shows that our policy outperforms the DNN-based recommender by about 4\% in total duration and nearly 7\% in the total number of click-throughs per-user-per-day.

We first explain how to eliminate outliers.
An outlier is typically introduced in two ways. 
In practice, users may accidentally swipe through two cards in a row, without even looking at the first one. 
We thus remove any \imp\ with duration less than $0.2$ seconds. 
On the other hand, users may sometimes leave their devices unattended for minutes, generating an abnormally high duration.
Since most cards' content can be fully consumed within 300 seconds, we remove any impression with duration over $u=300$ seconds.

\subsection{Analysis of $2^2 = 4$ Metrics}
\begin{table}[]
\caption{Types of Data In the Analysis}
\centering
\begin{tabular}{lll}
    & \multicolumn{1}{c}{CT} & \multicolumn{1}{c}{Duration} \\ \hline
Per User-Day   & \multicolumn{1}{c}{integral} & \multicolumn{1}{c}{numeric}  \\ \hline
Per Impression & \multicolumn{1}{c}{binary} & \multicolumn{1}{c}{numeric} \\ \hline
\end{tabular}
\label{tab:data_types}
\end{table}

The firm is interested in the analysis at the {\it per-user-per-day} and {\it per-\imp} levels, and two measures for user engagement: duration and click-throughs. 
So altogether we have {\bf four} metrics in total, as shown in Table~\ref{tab:data_types}.
% For each of these metrics,  we will later compare the the policies' performance using two basic statistical methods, the significance test and difference-in-difference (DID) test. 
In the per-\imp\ analysis, we treat each \imp\ as an \indep\ sample.
For example, the row for per-\imp\  duration in Table~\ref{tab:overall_stat} is the ratio between the total duration and total number of \imp s.
% Since the per-\imp\ conversion rate is what the Sieve policy learns, it will not be MAB group to outperform in terms of both mean duration and Click-Through Rate (CTR).

\begin{table}[]
\caption{Overall Statistics}
\centering
\begin{tabular}{lllllll}
& & & \multicolumn{2}{c}{May} & \multicolumn{2}{c}{July} \\ \cline{4-7}
& & & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{MAB} & \multicolumn{1}{c}{NN} & \multicolumn{1}{c}{MAB} \\ \hline
\multirow{5}{*}{Per-User-Per-Day} & \multirow{3}{*}{Duration} & Mean & 175.910 & 175.548 & 137.059 & 142.618 \\ \cline{3-7} 
& & SE Mean & 0.699 & 0.659 & 0.6081 & 0.597 \\ \cline{3-7}
& & Median  & 44.250 & 44.279 & 32.973 & 34.430 \\ \cline{2-7} 
& \multirow{2}{*}{\#CT} & Mean & 1.275 & 1.273 & 0.941 & 1.010 \\ \cline{3-7} 
 & & SE Mean & 9.251e-03 & 8.814e-03 & 7.276e-03 & 7.549e-03 \\ \hline
\multirow{5}{*}{Per Impression} & \multirow{3}{*}{Duration} & Mean    &   3.9697 & 4.0195 & 4.1183 & 4.2391\\ \cline{3-7} 
 & & SE Mean & 4.529e-03  & 4.402e-03 & 5.738e-03 & 5.599e-03 \\ \cline{3-7} 
 & & Median  & 0.693 & 0.697 & 0.702 & 0.703 \\ \cline{2-7} 
 & \multirow{2}{*}{CTR} & Mean    & 2.887e-02 & 2.915e-02 & 2.827e-02 & 3.001e-02 \\ \cline{3-7} 
 & & SE Mean & 4.698e-05 & 4.568e-05 &5.804e-05 & 5.671e-05 \\ \hline
\end{tabular}
\label{tab:overall_stat}
\end{table}

However, the firm's \obj\ is the {\bf total} user engagement rather than the {\it per-\imp} engagement, which motivated our analysis on the per-user-per-day level.
At first sight, it seems reasonable to consider the total engagement of a fixed user over {\bf all} 14 days during the experiment.
However, this metric is flawed since the frequency at which the users enter the app is affected by many external factors, such as holidays and weekends, which introduces extra noise.
% We thus group each user's \imp s by day as follows. 
We will thus only consider the days  when a user entered the app (i.e., has at least one \imp).
Formally, for each user $u$ and day $d$ where this user has at least one \imp,  we define a tuple $(u, d, D_{ud})$ where $D_{ud}$ is the total duration.
Thus, the number of tuples associated with  each  user is between $1$ and $14$. 

% Before providing the formal definition, we first explain why it is necessary to group the data by users and days \resp. 
% As we recall, the partition of control versus experimental group was randomly decided by Glance much earlier than the field experiment.
% In \parti, a portion of old users have left the platform, and thus the control and treatment groups have evolved to different sizes over time. 
% Therefore it is reasonable not to simply aggregate the user engagement in the two groups.

Under this definition of total engagement, we summarize\footnote{The unit of duration in all tables is {\it second}} the experimental results in Table~\ref{tab:overall_stat} and visualize the per-user-per-day user engagement in Figure \ref{fig:CT_per_user_per_day} and Figure \ref{fig:duration_per_user_per_day}.
% For both number of click-throughs and duration, 
We observe that in May the user engagement of the two groups are \apx ly identical, but in July the MAB group has a significantly higher mean user engagement.
Moreover, such improvement also appeared in {\it median} duration, indicating that this improvement is unlikely to be caused by a heavier tail in the \distr.

\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
\centering \includegraphics[width=\linewidth]{fig/_CT_per_user_day.png}
  \caption{Number of click-throughs per-user-per-day}  \label{fig:CT_per_user_per_day}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
 \includegraphics[width=\linewidth]{fig/_duration_per_user_day.png}
  \caption{Duration per-user-per-day}
\label{fig:duration_per_user_per_day}
\end{minipage}
\end{figure}

It is also worth noting that the user engagement per-user-per-day decreased from May to July. 
This is because May 2021 was when the Covid-19 pandemic reached its peak in the country where most users were located.
During the lockdown, the users may have had more time to spend on the app, resulting in a higher total engagement.
In Section \ref{sec:DID}, we perform a DID analysis which incorporates the underlying change of \env\ across time.

Finally we emphasize that in our implementation, our policy is {\bf not} personalized. 
Despite this  disadvantage, our Sieve policy still outperforms their  personalized DNN recommender in {\bf all}
metrics for user-engagement, both at the per-impression and per-user levels; see Table \ref{tab:overall_stat}.

\subsection{Significance Tests}\label{sec:DID}
From Figure \ref{fig:CT_per_user_per_day} and Figure \ref{fig:duration_per_user_per_day} we observe that our policy outperforms the control policy. 
We now test whether this improvement is statistically significant.

For each month $m \in$ \{May, July\}, denote by $X^m, Y^m$ the user engagement (either duration or number of click-throughs) in the NN and MAB group \resp.
Similarly, denote by $\overline{X}^m, \overline{Y}^m$ be the sample means of $X^m, Y^m$ in month $m$.
We are interested in the {\it difference-in-differences} in user engagement before and after our policy was deployed, i.e., 
\[\Delta = (Y^{\mathrm{July}}-X^{\mathrm{July}}) - (Y^{\mathrm{May}}-X^{\mathrm{May}}).\]
Consider the hypotheses
$$H_0 : \ho{E}[\Delta] \leq 0 \ \ \ \ \text{vs.}\ \ \  H_1: \ho{E}[\Delta] >0.$$ 
First consider the basic 
$Z$-score given by
\begin{align}
%\label{eqn:nov13a}
Z = 
\frac {\left(\overline{Y}^{\mathrm{July}} \overline{X}^{\mathrm{July}}\right) - \left(\overline{Y}^{\mathrm{May}}-\overline{X}^{\mathrm{May}}\right)}{\hat S}
\end{align}
where 
\begin{align*}
\hat S = \mathrm{SE} \left(\left(\overline{Y}^{\mathrm{July}}-\overline{X}^{\mathrm{July}}\right) - \left(\overline{Y}^{\mathrm{May}}-\overline{X}^{\mathrm{May}}\right)\right) = \sqrt{\mathrm{Var} \left(\left(\overline{Y}^{\mathrm{July}}-\overline{X}^{\mathrm{July}}\right) - \left(\overline{Y}^{\mathrm{May}}-\overline{X}^{\mathrm{May}}\right)\right)}
\end{align*}
is the estimated standard deviation.
For $Z\in \{ X^{\mathrm{May}}, X^{\mathrm{July}}, Y^\mathrm{May}, Y^\mathrm{July}\}$ we denote by
$N_Z$ the number of i.i.d. samples of $Z$, and let $S^2_Z$ be the sample variance.
Assuming the samples are \indep, we may approximate the above as 
\[\hat S \approx \sqrt{\frac 1{N_{X^\mathrm{May}}} S_{X^{\mathrm{May}}}^2 + \frac 1{N_{X^\mathrm{July}}} S_{X^{\mathrm{July}}}^2 + \frac 1{N_{Y^\mathrm{May}}} S_{Y^{\mathrm{May}}}^2 +\frac 1{N_{Y^\mathrm{July}}} S_{Y^{\mathrm{July}}}^2}.\]
As shown  in the ``Basic'' column of Table~\ref{tab:ht}, the $p$-values for each of the four metrics are very low. We therefore reject the null \hypo\ $H_0$ and conclude that the treatment effect is statistically significant.

\begin{table}[]
\centering
\caption{Significance Testing}
\begin{tabular}{llllll}
 & & \multicolumn{2}{c}{Basic} & \multicolumn{2}{c}{Bootstrap} \\ \cline{3-6} 
 & & \multicolumn{1}{c}{$Z$-score} & \multicolumn{1}{c}{$p$-value} & \multicolumn{1}{c}{$Z$-score} & \multicolumn{1}{c}{$p$-value} \\ \hline
\multirow{2}{*}{Per-User-Per-Day}   & Duration & 4.610 &2.018e-06 & 4.6197 & 1.921e-06 \\ \cline{2-6}
 & CT & 4.259 & 1.027e-05 & 4.2556 & 1.042e-05 \\ \hline
\multirow{2}{*}{Per Impression} & Duration & 6.963 & 1.665e-12 & 6.972 & 1.556e-12 \\ \cline{2-6} 
 & CT &12.999 & 6.127e-39 & 12.933 & 1.469e-38\\ \hline
\end{tabular}
\label{tab:ht}
\end{table}

However, in reality the samples are {\bf not} \indep, since (1) each user may appear in both months, (2) each user has multiple data points in a month, and (3) the same set of cards is shown to both the treatment and control group. 
% In fact, a user may have at most 14 data points in each group since the experiment lasted for 14 days.
We remove the dependence by bootstrapping as follows.
From each of these four sets of data points, we randomly draw $10^6$ samples with replacement and redefine each $\bar Z$ as the bootstrap sample mean where $Z= X^{\mathrm{May}}, X^{\mathrm{July}}, Y^{\mathrm{May}},Y^{\mathrm{July}}$;  see the ``Bootstrap'' column in Table \ref{tab:overall_stat}. 
We still observe very low $p$-values, which further validates our conclusion.
% The results with bootstrapping is consistent with our earlier findings, 

\subsection{DID Regression}
Now we consider a DID regression analysis. 
We first illustrate the idea of DID regression in Figure \ref{fig:DID} using the duration per impression as an example.
We first vectorize each tuple $(u,d,Y_{ud})$ into a four-dimensional vector $(t_{ud},i_{ud},t_{ud}\cdot i_{ud},Y_{ud})$ where 
\[t_{ud}={\bf 1}[\text{day } d \text{ is in July}] 
\quad \text{and} \quad i_{ud}={\bf 1}[\text{user } u \text{ is in MAB group}]\]
are the time and intervention  indicators, and $Y_{ud}\in \{C_{ud}, D_{ud}\}$ is the metric under consideration (i.e., click-throughs or duration of user $u$ on day $d$).
The basic assumption in a DID analysis is that the outcome follows the linear model
\begin{align}\label{eqn:nov12}
Y_{ud} = \beta_0 + \beta_1 t_{ud} + \beta_2 i_{ud} + \beta_3 t_{ud}\cdot i_{ud} + \eps_{ud}
\end{align}
where $\eps_{ud}\sim N(0,\sigma^2)$ with \unk\ variance $\sigma^2$.
Intuitively, $\beta_1$ measures the effect of being assigned to the treatment group and $\beta_2$ captures the overall trend over time.
Thus, if there is no treatment effect, the differences between the two groups should remain unchanged across May and July, and therefore the means of the samples from the four pools ({\it shown as the red dots} in Figure~\ref{fig:DID}) will form a perfect parallelogram.

Now \sps\ there is indeed a positive treatment effect. 
Then, the top-right corner of this quadrilateral will be raised; see the green dot in Figure~\ref{fig:DID}.
This lift is measured by the variable $\beta_3$.
To see this, by setting $t_{ud}=i_{ud}=0$, we observe that $\beta_0$ is  the mean engagement of control group users in May.
Further, note that the top-right corner of the parallelogram is $\beta_1 + \beta_2 + \beta_0$.
In contrast, for day $d$ in July and user $u$ in MAB group, if
$i_{ud} = t_{ud} = 1$, then the mean outcome \sats\ $\ho{E}[Y_{ud}] = \beta_0 + \beta_1 + \beta_2 + \beta_3$, which is higher than the top-right red dot by $\beta_3$.

\begin{figure}
\centering
 \includegraphics[width=0.6\linewidth]{fig/DID_022423.png}
\centering
 \caption{Illustration of DID regression {\new for  duration per \imp}}
 \label{fig:DID}
\end{figure}

Assuming the Gaussian noise, we are able to compute \ci s and $p$-values for the \coeff\ $\beta_i$'s; see  Tables \ref{tab:DID}.
For both duration and CT, the coefficients $\beta_3$ are positive and have very low $p$-values. 
Therefore, it is is indeed significant whether a user is assigned to the MAB group.
Moreover, note that $\beta_2$ has high $p$-values, so we conclude that the partition of users is sufficiently random, at least on the per-user-per-day level.

As shown in the second half of Table~\ref{tab:DID}, we also consider per-\imp\ user engagement.
Similar to the above analysis, we convert each \imp\ $j$ into a three-dimensional binary vector $(t_j, i_j, Y_j)$ where $Y_j$ is either the duration  or click-through indicator  for \imp\ $j$.
Note that the duration per \imp\ is numerical so we can analyze it using linear regression \eqref{eqn:nov12}. 
In contrast, the per \imp\ click-throughs $(Y_j)$ are {\it binary}, so we instead apply logistic regression: we assume  $Y_j \sim \mathrm{Ber}\left(\frac {e^z}{1+e^z}\right)$ where 
\[z = \beta_0 + \beta_1 t_j + \beta_2 i_j + \beta_3 t_j i_j.\]

As opposed to the per-user-per-day regression, in this case {\bf all} coefficients have tiny $p$-values for both CT and duration.
In \parti, the coefficient $\beta_2$ for intervention has low $p$-value, indicating that the initial user partition may not be truly random in terms of per \imp\ engagement.
Nonetheless, this difference is interpretable: our experiment was performed on random user-groups that Glance has been using for months prior to our field test, on which some previous experiments have been performed, causing this discrepancy in user behavior. 

We next quantify the improvement. 
For the per-user-day conversion, we observe that the total duration and the number of click-throughs improved by $\beta_3/(\beta_0+\beta_1)\approx 4.319\%$ and $7.482\%$ \resp.
For the per impression conversion, the duration improved by $1.726\%$.
Finally, note that the $\beta$'s for CTR are based on {\it logistic} regression. 
The improvement {\new in the odds ratio} is $e^{\beta_3}-1\approx 4.854\%.$

\begin{table}[]
\centering
\caption{Difference-In-Differences Regression}
\label{tab:DID}
\begin{threeparttable}
\begin{tabular}{lllcccccc}
%\begin{tabular}{lllllllll}
 & & & Coef. & Std. Dev. & $t$ & $p$-value & 0.025Q & 0.975Q \\ \hline
\multirow{8}{*}{Per User-Day}   & \multirow{4}{*}{Duration} & $\beta_0$ & 175.9103 & 0.640    & 274.941 & 0.000   & 174.656 & 177.164 \\ \cline{3-9} 
 & & $\beta_1$ & -38.8514 & 0.942    & -41.263 & 0.000   & -40.697 & -37.006 \\ \cline{3-9} 
 & & $\beta_2$ & -0.3622  & 0.887    & -0.409  & 0.683   & -2.100  & 1.375           \\
 \cline{3-9} 
 & & $\beta_3$ & {\bf 5.9208}   & 1.303 & 4.544   & {\bf 2.759e-06}   & 3.367   & 8.475  \\ \cline{2-9} 
 & \multirow{4}{*}{\#CT}       & $\beta_0$ & 1.2750  & 0.008    & 153.851 & 0.000   & 1.259  & 1.291 \\ \cline{3-9} 
 & & $\beta_1$ & -0.3341 & 0.012 & -27.394 & 1.616e-165 & -0.358 & -0.310 \\ \cline{3-9} 
 & & $\beta_2$  & -0.0016 & 0.011 & -0.141  & 0.888 & -0.024 & 0.021  \\ \cline{3-9} 
 & & $\beta_3$ & {\bf 0.0704}  & 0.017 & 4.171 & {\bf 1.516e-05} & 0.037  & 0.103 \\ \hline
\multirow{8}{*}{Per Impression} & \multirow{4}{*}{Duration} & $\beta_0$ & 3.9697& 0.005& 863.796 & 0.000& 3.961& 3.979\\ \cline{3-9} 
& & $\beta_1$ & 0.1486 & 0.007 & 20.234 & 2.753e-89 & 0.134& 0.163\\ \cline{3-9} 
& & $\beta_2$ & 0.0497 &0.006 & 7.781& 3.597e-15 & 0.037& 0.062 \\ \cline{3-9} 
& & $\beta_3$ & {\bf 0.0711} & 0.010 & 6.998 & {\bf 1.298e-12} & 0.051& 0.091\\ \cline{2-9} 
& \multirow{4}{*}{CTR} & $\beta_0$ & -3.5198 & 0.002 & -2092.794 & 0.000 & -3.523 & -3.517\\ \cline{3-9} 
& & $\beta_1$ & -0.0161 & 0.003 & -5.947 & 1.365e-09 & -0.021 & -0.011 \\ \cline{3-9} 
& & $\beta_2$ &  0.0133 & 0.002 & 5.712 & 5.582e-09 & 0.009 & 0.018\\ \cline{3-9} 
& & $\beta_3$ & {\bf 0.0474} & 0.004 & 12.819 & {\bf 6.417e-38} & 0.040 & 0.055 \\ \hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item Note: All regression are linear regression except for per \imp\ CT, where we applied logistic regression due to binary labels.
    \end{tablenotes}
  \end{threeparttable}
\end{table}

\iffalse
\subsection{Analysis For Engaged Users}\label{subsec:user_subset}
In this subsection we analyze the engagement of special subsets of ``engaged'' users.
We first consider the retention rate from May to July. 
A user is said to be {\it engaged} in month $m\in \{$May, July\} if she has at least $k$ click-throughs in month $m$. 
The attrition rate (for NN and MAB group \resp) is then defined to be the proportion of engaged users in May who remained engaged in July.
While there is no obvious choice for the threshold $k$, Figure~\ref{fig:attrition} shows that for each  $k=1,2,...,10$, the attrition rates of the MAB group is consistently higher than the NN group, which suggests that the choice of $k$ is likely not essential.
Thus, in the remaining analysis we will fix this threshold to be $k=4$ and repeat the analysis in Section~\ref{subsec:all_user}.

By comparing Table~\ref{tab:overall_stat} and \ref{tab:overall_stat_engaged}, we observed that for engaged users, both the per-user-per-day duration and click-throughs are notably higher than the average over all users, indicating that our definition for ``engaged'' user indeed captures the enthusiasm of users.
As another noteworthy observation, for each of the four DID regressions in Table~\ref{tab:DID} and \ref{tab:DID_engaged}, the coefficient $\beta_3$ for the magnitude of the composite variable is higher for the engaged users than for all users.
This suggests that the treatment effect is even more significant for the engaged users. 

\begin{table}[]
\centering
\caption{Overall Statistics For Engaged Users}
\begin{tabular}{lllllll}
 & & & \multicolumn{2}{c}{May} & \multicolumn{2}{c}{July} \\ \cline{4-7}
 & & & NN         & MAB        & NN         & MAB         \\ \hline
\multirow{5}{*}{Per User-Day}   & \multirow{3}{*}{Duration} & Mean    & 404.707 & 403.228 & 303.002 & 314.272 \\ \cline{3-7} 
& & SE Mean &2.142 & 2.010 & 2.670 & 2.496\\ \cline{3-7} 
& & Median  & 196.970 & 199.845 & 133.348 & 146.230 \\ \cline{2-7} 
& \multirow{2}{*}{\#CT} & Mean & 4.235 & 4.236 & 2.657 & 2.866\\ \cline{3-7} 
& & SE Mean & 3.241e-02 & 3.080e-02 & 3.642e-0s2 & 3.661e-02\\ \hline
\multirow{5}{*}{Per Impression} & \multirow{3}{*}{Duration} & Mean & 3.790 & 3.866 &3.659 & 3.850 \\ \cline{3-7} 
 & & SE Mean & 5.922e-03 & 5.802e-03 & 1.022e-02 & 1.076e-02 \\ \cline{3-7} 
 & & Median  & 0.619 & 0.622 & 0.594 & 0.598 \\ \cline{2-7} 
& \multirow{2}{*}{CTR} & Mean    & 3.954e-02 & 4.043e-02 & 3.198e-02 & 3.498e-02 \\ \cline{3-7} 
 & & SE Mean & 6.802e-05 & 6.671e-05 & 1.074e-05 & 1.062e-05 \\ \hline
\end{tabular}
\label{tab:overall_stat_engaged}
\end{table}

\begin{table}[]
\centering
\caption{Significance Testing For Engaged Users}
\begin{tabular}{llllll}
& & \multicolumn{2}{c}{Basic} & \multicolumn{2}{c}{Bootstrap} \\ \cline{3-6} 
& & \multicolumn{1}{c}{$Z$-score} & \multicolumn{1}{c}{$p$-value} & \multicolumn{1}{c}{$Z$-score} & \multicolumn{1}{c}{$p$-value} \\ \hline
\multirow{2}{*}{Per User-Day}   & Duration & 2.719 & 3.273e-03 & 2.717 & 3.289e-03 \\ \cline{2-6} 
 & \#CT &3.056  & 1.121e-02 & 3.064 & 1.089e-02 \\ \hline
\multirow{2}{*}{Per Impression} & Duration & 6.996 &  1.321e-12 & 7.060  & 8.301e-13 \\ \cline{2-6}
& CTR & 11.626 &1.513e-31 & 11.478 & 8.482e-31 \\ \hline
\end{tabular}
\end{table}


\begin{figure}
\centering
\begin{minipage}{.5\textwidth}
  \centering
  \includegraphics[width=\linewidth]{fig/retention_rate.png}
  \caption{Attrition rates of the MAB and NN group.}
  \label{fig:attrition}
\end{minipage}%
\begin{minipage}{.5\textwidth}
  \centering
\includegraphics[width=\linewidth]{fig/duration_user_day.png}
  \caption{Duration per user-day pair.}
  \label{fig:test2}
\end{minipage}
\end{figure}

\begin{table}[]
\caption{Difference-In-Differences Regression for Engaged Users}
\label{tab:DID_engaged}
\begin{threeparttable}
\begin{tabular}{lllcccccc}
                 & &           & Coef. & Std. Dev. & $t$ & $p$-value & 0.025Q & 0.975Q \\ \hline
\multirow{8}{*}{Per User-Day}   & \multirow{4}{*}{Duration} & $\beta_0$ & 404.7074 & 2.008 & 201.569 & 0.000 & 400.772 & 408.643\\ \cline{3-9} 
 & & $\beta_1$ &  -101.7057 & 3.692 & -27.548 & 2.338e-167 & -108.942 & -94.470\\ \cline{3-9} 
 & & $\beta_2$ &  -1.4791 & 2.782 & -0.532 & 0.595 & -6.932 & 3.974\\ \cline{3-9} 
 & & $\beta_3$ & 12.7489 & 5.083 & 2.508 & 0.012 & 2.786 & 22.711 \\ \cline{2-9} 
 & \multirow{4}{*}{CT}       & $\beta_0$ & 4.2353 & 0.030 & 140.602 & 0.000 & 4.176 & 4.294 \\ \cline{3-9} 
 &                           & $\beta_1$ & -1.5787 & 0.055 & -28.502 & 5.532e-179 & -1.687 & -1.470\\ \cline{3-9} 
 &                           & $\beta_2$ & 0.0006 & 0.042 & 0.015 & 0.988 & -0.081 & 0.082\\ \cline{3-9} 
 &                           & $\beta_3$ & 0.2086 & 0.076 & 2.736 & 0.006 & 0.059 & 0.358\\ \hline
\multirow{8}{*}{Per Impression} & \multirow{4}{*}{Duration} & $\beta_0$ &  3.7789 & 0.006 & 634.095 & 0.000 & 3.767 & 3.791 \\ \cline{3-9} 
 & & $\beta_1$ &  -0.131 & 0.012 & -10.854 & 9.544e-28 & -0.154 & -0.107  \\ \cline{3-9} 
& & $\beta_2$ &  0.0723 & 0.008 & 8.708 & 1.546e-18 & 0.056 & 0.089  \\ \cline{3-9} 
& & $\beta_3$ & 0.1162 & 0.017 & 6.998 & 1.298e-12 & 0.084 & 0.149 \\ \cline{2-9} 
& \multirow{4}{*}{CT} & $\beta_0$ & -3.190 & 0.002 & -1771.359 & 0.000 & -3.193 & -3.186\\ \cline{3-9} 
& & $\beta_1$ &  -0.220 & 0.004 & -55.949 & 0.000 & -0.228 & -0.212  \\ \cline{3-9} 
 & & $\beta_2$ &   0.0237 & 0.002 & 9.500 &  1.049e-21 & 0.019 & 0.029  \\ \cline{3-9} 
 & & $\beta_3$ & 0.0691 & 0.005 & 12.942 & 1.303e-38 & 0.059 & 0.080 \\ \hline
\end{tabular}
    \begin{tablenotes}
      \small
      \item Note: As in the previous section, all regression are linear regression except for per \imp\ CT, where we applied logistic regression due to binary labels.
    \end{tablenotes}
  \end{threeparttable}
\end{table}
\fi
